DISAPERE: A Dataset for Discourse Structure in Peer Review Discussions

At the foundation of scientific evaluation is the labor-intensive process of peer review. This critical task requires participants to consume vast amounts of highly technical text. Prior work has annotated different aspects of review argumentation, but discourse relations between reviews and rebuttals have yet to be examined. We present DISAPERE, a labeled dataset of 20k sentences contained in 506 review-rebuttal pairs in English, annotated by experts. DISAPERE synthesizes label sets from prior work and extends them to include fine-grained annotation of the rebuttal sentences, characterizing their context in the review and the authors' stance towards review arguments. Further, we annotate every review and rebuttal sentence. We show that discourse cues from rebuttals can shed light on the quality and interpretation of reviews. Further, an understanding of the argumentative strategies employed by the reviewers and authors provides useful signal for area chairs and other decision makers.

==> 01_old_intro.tex <==
\section{Introduction}

Peer review performs the essential role of quality control in the dissemination of scientific knowledge. The rapid increase in academic output places an immense burden on decision makers such as area chairs and editors, as their decisions must take into account not only extensive manuscripts, but enormous additional amounts of technical text including reviews, rebuttals, and other discussions.

Many proposed solutions to peer review's shortcomings require systemic change and institutional buy-in across international communities \citep{church-rther, nobarany_rethinking_2014, ko_modern_2019}. However, an understanding of the interaction between participants in the discussion is more easily achieved and would be valuable to any such effort. Prior work has annotated various properties of peer review text. We present \textbf{\myname} (DIscourse Structure in Academic PEer REview), a dataset synthesizing and extending these annotation schemes to surface a rich characterization of this interaction. \Cref{fig:mainfig} shows the \myname annotation scheme on a minimal, fictional example review-rebuttal pair.


Most peer review formats allow authors to respond to the reviewers' comments in a \textit{rebuttal}. We argue that the discourse structure of the rebuttal can be particularly instructive to observers of the peer review process, providing additional context on the quality and interpretation of the reviews. To achieve this, we annotate each sentence of a rebuttal with a fine-grained label indicating the author's intentions and commitment, and a link to the set of review sentences that form its context. The review sentences, in turn, are each annotated with four types of labels providing a detailed view of the context of the rebuttal.

\myname is intended as a comprehensive and high-quality test collection, along with training data to fine-tune models.  Our annotations are carried out by graduate students in computer science who have undergone training and calibration, amounting to over 850 person-hours of annotation work. Much of the test data is double-annotated, and we report inter-annotator agreement on all aspects of the annotation. We believe that this dataset can support varied research questions in the area of peer review, while also enabling the construction of practical tools for peer reviewers and decision makers. We present one example in which information from our annotations can directly benefit area chairs of a conference. Introducing the concept of \textit{agreeability} \pcref{sec:application}, we show that measuring the extent to which authors agree with the premises of reviewers' criticisms can be used to locate problematic forums that require area chairs' intervention.

Prior work casts peer review as an argumentative task, focusing on arguments made in the manuscript and reviewers and authors' stances towards these arguments. This precludes study of participants' adherence to social norms and unspoken expectations, such as that of providing a summary, of being concise and polite, and of being constructive \citep{glonti2019scoping}. By annotating \textit{every} sentence in the review and the rebuttal, we allow researchers to access these non-argumentative properties of the peer review texts beyond the purview of conventional argument types.


The contributions of this paper are as follows:
(1) a new labeled training dataset of 506 review-rebuttal pairs (over 20k sentences) of peer review discussion text in English;
(2) a taxonomy of discourse labels synthesizing prior work on discourse in peer review and extending it to add useful subcategories;
(3) a summary of the performance of baseline models on this dataset, and
(4) annotation software and extensive annotation guidelines to support future labeling efforts in this area. 


==> tables/01_fig_table.tex <==


\begin{table*}[]
{\scriptsize %  
\begin{tabular}{|l|l|l|l|p{0.3\linewidth}|lll|p{0.3\linewidth}|l|}
\cline{1-5} \cline{9-10}
\makecell{Review \\ action}
	& \makecell{Fine rev. \\ action}
	& Asp.
	& Pol.
	& Review (by Reviewer 1)
	& & &
	& Rebuttal (by Authors)
	& \makecell{Rebuttal \\ action} \\ \cline{1-5} \cline{9-10} 

Struct.
	& Summ.
	& - 
	& o 
	&This paper proposes a simple, but effective technique.
	& \tikzmark{rev1} & & \tikzmark{reb1}
	& \multirow{2}{\linewidth}{We are grateful for the suggestions that have contributed significantly to the paper’s quality.}
	& \multicolumn{1}{c|}{\multirow{2}{*}{ Social}} \\ \cline{1-5}

Eval.
	& -
	& SUB 
	& +
	& The idea is intuitive and justified by their theoretical analysis.
	& \tikzmark{rev2} & & \tikzmark{reb2}
	& &                         \\ \cline{1-5} \cline{9-10} 

Eval.
	& -
	& CLA
	& +
	& The paper is well-written and easy to understand.
	& \tikzmark{rev3} & & 
	& We thank the reviewer for recognizing our theoretical contributions.
	& \makecell{Accept\\ praise}           \\ \cline{1-5} \cline{9-10} 

Eval.
	& -
	& CLA
	& -
	& It would be helpful to note in the description of Table 3 what is better (higher/lower).
	& \tikzmark{rev4} & & \tikzmark{reb3}
	& Being a new problem setting, designing appropriate baselines can be challenging.
	& \makecell{Mitigate\\ criticism}      \\ \cline{1-5} \cline{9-10} 

Eval.
	& -
	& CMP
	& -
	& A proper baseline should have been compared.
	& \tikzmark{rev5} & & \tikzmark{reb4}
	& But we agree with most of the criticisms.
	& \makecell{Concede\\ criticism}       \\ \cline{1-5} \cline{9-10} 

Req.
	& \makecell{Add\\ expt.}
	& -
	& o
	&Results on data from other domains will make the performance more convincing.
	& \tikzmark{rev6} & & \tikzmark{reb5}
	& Please refer to our updated “Experiments” section for results on more domains.
	& \makecell{Task\\ done}               \\ \cline{1-5} \cline{9-10} 
\end{tabular}
}
\begin{tikzpicture}[overlay, remember picture, shorten >=.5pt, shorten <=.5pt, transform canvas={yshift=.25\baselineskip}]
    \draw [->] ({pic cs:reb2}) to ({pic cs:rev2});
    \draw [->] ({pic cs:reb3}) to ({pic cs:rev4});
    \draw [->] ({pic cs:reb3}) to ({pic cs:rev5});
    \draw [->] ({pic cs:reb3}) to ({pic cs:rev6});
    \draw [->] ({pic cs:reb4}) to ({pic cs:rev5});
    \draw [->] ({pic cs:reb5}) to ({pic cs:rev6});
    %\draw [->] ([yshift=.75pt]{pic cs:reb2}) -- ({pic cs:rev1);
  \end{tikzpicture}
\end{table*}

